CoSA: Scheduling by Constrained Optimization for Spatial Accelerators

Recent advances in Deep Neural Networks (DNNs) have led to active development of specialized DNN accelerators, many of which feature a large number of processing elements laid out spatially, together with a multi-level memory hierarchy and flexible interconnect. While DNN accelerators can take advantage of data reuse and achieve high peak throughput, they also expose a large number of runtime parameters to the programmers who need to explicitly manage how computation is scheduled both spatially and temporally. In fact, different scheduling choices can lead to wide variations in performance and efficiency, motivating the need for a fast and efficient search strategy to navigate the vast scheduling space. To address this challenge, we present CoSA, a constrained-optimization-based approach for scheduling DNN accelerators. As opposed to existing approaches that either rely on designers' heuristics or iterative methods to navigate the search space, CoSA expresses scheduling decisions as a constrained-optimization problem that can be deterministically solved using mathematical optimization techniques. Specifically, CoSA leverages the regularities in DNN operators and hardware to formulate the DNN scheduling space into a mixed-integer programming (MIP) problem with algorithmic and architectural constraints, which can be solved to automatically generate a highly efficient schedule in one shot. We demonstrate that CoSA-generated schedules significantly outperform state-of-the-art approaches by a geometric mean of up to 2.5x across a wide range of DNN networks while improving the time-to-solution by 90x.

==> 7codesign.tex <==
\section{Case Study: On-chip Memory Partitioning with~\sys{}}
\label{sec:allocation} 
In addition to scheduling for a given hardware, due to the fast, one-shot nature of \sys{}, it can also be applied for hardware and scheduling co-design problem.
In particular, on-chip memory partitioning is a critical design decision that can greatly impact not only the overall area budget but also the scheduling decision, especially in architectures with multi-level private buffers for different data tensors. 
Given an on-chip memory budget, the memory partitioning algorithm determines the portion of memory to assign to each local buffer. 
% Lacking a mature scheduler that efficiently maps the target workload onto a multi-level memory hierarchy, 
% the design space exploration for SRAM partitioning may lead to sub-optimal solutions. 
% \sys, on the other hand, generates high-quality schedules for each hardware design point, which helps to better navigate the search space for memory partitioning.
Current work on the design space exploration of accelerators for resource allocation~\cite{timeloop2019-ispass, interstellar-asplos2020, kao20confuciux, choi2020dance, zhang2020dna} rely on the iterative scheduling schemes that are computationally expensive and can yield sub-optimal solutions. 
%For the on-chip memory partitioning problem targeted by our work, existing methods use analytical optimization~\cite{zidenberg2012multiamdahl}~\cite{morad2012generalized} without considering the impact of scheduling.
Our work is the first work that formulates both the scheduling decisions and the on-chip memory partitioning problem as a single optimization problem.
%% FPGA 
%FPGA scheduling with memory partitioning \cite{cong2011automatic}
%embedded system SoC task scheduling and memory partitioning ~\cite{niemann1996hardware, benini2005allocation, salamy2012effective}.
%To the best of our knowledge, there is no prior work that formulates both the scheduling decisions and the on-chip memory partitioning problem into one optimization and directly solves them towards a given performance objective.  
\subsubsection{Formulation}
To co-optimize the scheduling and memory partitioning decisions, we  modify the formulations in Section~\ref{sec:framework} to include memory sizes also as \sys variables.
Instead of treating the log capacity $log(M_{I,v})$ for different buffers as constraints in Section~\ref{sec:buf_util}, 
we turn them into MIP variables $m_{I,v}$ that represents the $\log$ value of the actual buffer size $w_{I,v}$. 
%o be solved in ~\sys{}. 
Assume we have $H$ on-chip buffers, 
we then need to add another constraint to ensure the total size of all buffers does not exceed the allocated budget $G$:
%The constraint can be formulated as follows:
\begin{equation}
\begin{aligned}
\sum^{H-1}_{I=0}\sum^{2}_{v=0} w_{I,v} = \sum^{H-1}_{I=0}\sum^{2}_{v=0} 2^{m_{I,v}} \le G
\end{aligned}
\end{equation} 
%However, since above constraint cannot be turned to a linear function of the log variable $m_{I,v}$, 
%this formulation cannot be directly solved by the constraint solver. 

%\subsubsection{Numerical Solver}
%As a workaround, we resort to a numerical iterative process to test for a maximum coefficient $\alpha \in [0,1]$, such that: 
%\begin{equation}
%\begin{aligned}
%&\sum^{H-1}_{I=0}\sum^{2}_{v=0} m_{I,v} \le \alpha (3H\log(G)-3H\log(3H)) \\
%&\sum^{2}_{v=0} 2^{m_{I,v}} \le G
%\end{aligned}
%\end{equation} 

%Note that the upperbound constant $3H\log(G)-3H\log(3H)$ %multiplied by $\alpha$ 
%is derived from 
%the concave  property of the $\log$ function.
%:  $\frac{\sum^{H-1}_{I=0}\sum^{2}_{v=0}\log(w_{I,v})}{3H} \le \log(\frac{\sum^{H-1}_{I=0}\sum^{2}_{v=0} w_{I,v}}{3H})$, where $\log(w_{I,v})=m_{I,v}$ and $\sum^{2}_{v=0} w_{I,v}=G$. 
% $ \frac{\sum^{Q-1}_{I=0}\sum^{2}_{v=0}m_{I,v}}{3Q} = \frac{\sum^{Q-1}_{I=0}\sum^{2}_{v=0}\log(w_{I,v})}{3Q} \le
% \log(\frac{\sum^{Q-1}_{I=0}\sum^{2}_{v=0} w_{I,v}}{3Q}) = \log(Z)-\log(3Q)$
%A bisection search is then performed to find the maximal $\alpha$ that satisfies the constraints above and solve for the corresponding $m_{I,v}$. % that represents the $\log$ size of each buffer.
%If the optimal $\sum^{H-1}_{I=0}\sum^{2}_{v=0} m_{I,v}$ is an increasing function of $\alpha$, the solutions should be close to optimal. For the objective functions in~\sys{}, especially the utilization objective $\hat{Util}$, larger total capacity allows for higher utilization and better performance. Therefore, a higher $\alpha$ should lead to a more optimal $m_{I,v}$. 

\subsubsection{Evaluation on On-chip Memory Partitioning}

\begin{figure}[t]
\begin{subfigure}[t]{0.48\columnwidth}
  \includegraphics[width=1\linewidth]{figs/sram_part_alexnet.pdf}
%   \vspace{10pt}
%   \includegraphics[width=0.97\linewidth]{figs/experiment_real_simba.pdf}
  \caption{\small \sys-generated memory partitions for AlexNet layers.
  }
  \label{fig:sram_part}
\end{subfigure}
\hspace{1pt}
\begin{subfigure}[t]{0.48\columnwidth}
  \includegraphics[width=1\linewidth]{figs/sram_part_sim_cycle.pdf}
%   \vspace{10pt}
%   \includegraphics[width=0.97\linewidth]{figs/experiment_real_simba.pdf}
  \caption{\small Speedup on hardware with \sys-generated memory partitions for AlexNet layers.
  }
  \label{fig:sram_sim_cycle}
\end{subfigure}
\end{figure}
%As we mentioned in Section~\ref{}.
Co-optimizing hardware and schedule opens up new optimization opportunities to balance different tradeoffs not only in the scheduling space but also in the hardware design.
As a starting point, we demonstrate how \sys{} can be extended to capture the design and scheduling tradeoffs.
In particular, 
%Since more optimization opportunities are exposed with the memory size constraints relaxed, we expect the latency performance to be better than the baseline result where schedules are generated based on a fixed evenly-distributed memory partitioning. 
Figure~\ref{fig:sram_part} shows the on-chip memory partitions solved by \sys for each layer in AlexNet. We observe significantly different preferred partitions for different layers, where some partition leads to up to 85\% reduction in the total SRAM size.
At the same time, Figure~\ref{fig:sram_sim_cycle} shows the corresponding performance % and energy 
of running each layer with \sys-generated schedules on the co-optimized hardware design. 
We see a 11\% improvement in the geomean speedup on the co-optimized hardware.
This case study shows a promising application of \sys in hardware-software codesign. 
\sys can be further extended to co-optimize other hardware design decisions by relaxing the architectural constraints in a similar manner as illustrated in this case study. 

==> ExtendedAbstract.tex <==
\title{\sys: Scheduling by Constraint Solvin for Spatial Accelerators}

\maketitle


\section{Motivation}
Recent advances in Deep Neural Networks (DNNs) have led to active development of
specialized DNN accelerators, many of which feature a large number of processing
elements laid out spatially, together with a multi-level memory hierarchy and
flexible interconnect.
While DNN accelerators improve the peak throughput and data reuse
opportunities, they also expose a large number of runtime parameters to the
programmers where programmers need to explicitly manage how computation is
scheduled both \textit{spatially} and \textit{temporally}.
In fact, different scheduling choices could lead to widely varying performance
and efficiency differences, motivating the need for fast and efficient
search strategy to navigate the vast scheduling space.

\section{Limitations of the State of the Art}
Given how a mapspace for a single DNN layer can be extremely large ($\sim$ billions of valid schedules), finding the optimal schedule can quickly become an intractable problem. State-of-the-art schedulers tackle this complexity mainly using one of the following two approaches. First, many schedulers resort to exhaustive search ~\cite{parashar2019timeloop, dave2019dmazerunner,yang2020interstellar,chatarasi2020marvel}. 
Such an approach is rendered viable because the scheduler starts with pruning the mapspace based on both the hardware and convolutional layer constraints. Disadvantages of this approach are two-fold: not only does such a brute-force search tend to be exceedingly expensive for more complex hardware architectures, but the generated schedules often do not perform optimally since analytical models fail to accurately capture the communication latency across the NoC.

Another class of current schedulers uses machine learning (ML) algorithms or other statistical methods ~\cite{chen2018tvm, ragan2013halide, jia2019_flexflow} to either improve the accuracy of the cost model or directly solve for the solution using blackbox-tuning. However, their computational costs can significantly outweigh their possible improvements in the generated schedule. (TBD) To-date, none of the schedulers following this approach have been able to address all three loop transformations we have proposed.

\section{Key Insights}
To address the large search space in the scheduling problem and the inefficiency in existing search strategies, we present \sys, a constraint-solver-based approach
for scheduling DNN accelerators.
Different from existing approaches that either rely on designers' heuristics or
expensive iterative methods to prune the search space, the key idea of \sys is
to formulate the scheduling decisions into a constraint-satisfaction problem
that can be deterministically solved using constraint solvers.
In particular, \sys leverages the regularities in DNN operators and hardware to
formulate the DNN scheduling space into a mixed integer programming problem with
algorithmic and architectural constraints, where it can automatically generate
a highly efficient schedule in a single pass.
%cosa results
We demonstrate that \sys-generated schedules significantly outperform
state-of-the-art approaches by \fixme{2}$\times$ across a wide range of DNN
networks while reducing the time-to-solution by \fixme{10}$\times$.

\section{Framework}
\sys{} targets the scheduling optimizations at the operation-level for mapping DNN workloads onto spatial accelerators. Similar to other standard constraint-solving-based frameworks, it consists of:
\begin{enumerate}[leftmargin=.4in]
    \item program and architecture dependent constraints
    \item decision variables to solve for
    \item objective functions
\end{enumerate}
It then optimizes the objective function subject to the constraints.  
\noindent
\subsection{\sys{} Variables} 
\sys{} takes the specifications of the DNN layers and the underlying spatial accelerator as input constraints and generates a valid schedule that is optimized towards the objective function. \sys{} makes three optimization decisions during the scheduling process:
\begin{enumerate}

\item \textbf{Loop Tiling} is a critical optimization to exploit the parallelism and data locality in a schedule. In Fig.~\ref{fig:tilling_characterization} of section~\ref{sec:bg_motivation}, we show that by only varying the tiling factors of a schedule, it can lead to up to 7$\times$ difference in performance. 
\item \textbf{Loop Permutation} affects the ordering of the outer temporal loop dimensions and changes the reuse patterns for different tensors. 
Loop permutation on a particular layer schedule alone can cause $\sim$30\% performance difference on our SystemC-based NoC simulator. 
\item \textbf{Spatial Mapping} determines whether to leverage spatial resources to parallelize the workload. Parallelization reduces the overall compute latency, however there is always a communication cost involved when mapping to spatial resource on a spatial NoC-based accelerator. Our framework aims to expose the search space for choosing a spatial dimension as well as determine to what extent we would like to parallelize each dimension as these also affects the traffic patterns on the NoC-based system.  
\end{enumerate}
\noindent
These three different optimizations should be co-optimized in one pass as they are interdependent. Decision made with each optimization will prune the search space for the others and the final performance gain in the optimization phase is not a linear combination of each optimization. 

\subsection{\sys{} Constraints} 
\begin{enumerate}

\item \textbf{Buffer Utilization}

\item \textbf{Spatial Resource Usage}
\end{enumerate}

\subsection{\sys{} Objective Functions} 
\begin{enumerate}

\item \textbf{Utilization-Driven Objective}

\item \textbf{Traffic-Driven Objective}

\item \textbf{Compute-Driven Objective}

\end{enumerate}

\section{Methodology}

\section{Key Results and Contributions}

\section{Why ASPLOS}

\section{Citation for Most Influential Paper Award}


==> figs/timeloop_listing.tex <==
\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  frame=L,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  frame=L,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
}

\lstset{escapechar=@,style=customc}

\begin{lstlisting}[frame=single, basicstyle=\tiny] 
-------------------------------------
| for P in [0:4)
GlobalBuffer [ Inputs:16384 Outputs:65536 ]
-------------------------------------------
|   for N in [0:1)
|     for K in [0:4) (Spatial-X)
|       for C in [0:4) (Spatial-X)
InputBuffer [ Inputs:4096 ]
---------------------------
|         for Q in [0:16)
|           for K in [0:8) (Spatial-Y)
WeightBuffer [ Weights:2048 ]
-----------------------------
|             for C in [0:8)
AccumulationBuffer [ Outputs:128 ]
----------------------------------
|               for K in [0:32)
|                 for C in [0:8) (Spatial-Y)
Registers [ Weights:1 ]
-----------------------
|                   for P in [0:4)
\end{lstlisting}
